GSGFormer: Generative Social Graph Transformer for Multimodal Pedestrian Trajectory Prediction

Pedestrian trajectory prediction, vital for selfdriving cars and socially-aware robots, is complicated due to intricate interactions between pedestrians, their environment, and other Vulnerable Road Users. This paper presents GSGFormer, an innovative generative model adept at predicting pedestrian trajectories by considering these complex interactions and offering a plethora of potential modal behaviors. We incorporate a heterogeneous graph neural network to capture interactions between pedestrians, semantic maps, and potential destinations. The Transformer module extracts temporal features, while our novel CVAE-Residual-GMM module promotes diverse behavioral modality generation. Through evaluations on multiple public datasets, GSGFormer not only outperforms leading methods with ample data but also remains competitive when data is limited.

==> sections/approach.tex <==
%!TEX root = ../main.tex
\section{Theoretical Approach} \label{sec:approach}


\subsection{Problem formulation}

% This part has been rewritten by Pavan 

Our problem of multimodally predicting pedestrian trajectories can be formally prescribed as follows. Starting with a bird's eye view (BEV) scene of an environment captured in RGB, semantically segmented into different classes, denoted by $\mathcal{M}$ contains a history of positions of each pedestrian in this scene. For each scene, there exist a finite number of goals that can be reached by a pedestrian denoted by $\mathcal{G}$. Each pedestrian also interacts with every other agent in the scene, denoted by $\mathcal{E}$. 

Given this information, the model aims to predict the distribution of pedestrian's trajectory for $H$ timesteps in the future.
% , denoted by $t_H$
%  denoted by $\mathbf{X}$
%

We aim to predict the distribution of the future trajectory based on all the history information we have, and then generate multi-modal trajectories for each agent. We learn the parameters $\theta$ of the probability $P_\theta(\mathbf{Y}|\mathbf{X})$ using a deep neural network model where $\mathbf{X}$ and $\mathbf{Y}$ are the input and output of the model.

Following the pedestrian trajectory prediction problem convention, the spatial coordinates of all the agents at different time stamps have been annotated initially. For the agent $i$, the model outputs the predicted future positions in the next $H$ time steps for current time $t$, which is represented as $\mathbf{Y}_i=(\mathbf{Y}_i^{t+1}, \mathbf{Y}_i^{t+2},... , \mathbf{Y}_i^{t+H})$. $\mathbf{Y}_i^t=(x_i^t, y_i^t)$ is the position coordinate of the agent. The input of the model is the history information in the past $n$ time steps, which can be denoted as $\mathbf{X}_i=(\mathbf{X}_i^{t-n+1}, \mathbf{X}_i^{t-n+2},... , \mathbf{X}_i^{t})$. In order to consider the effect of social forces, the history states of ego agent and all neighbors as well as the semantic map information are input to the model. We assume that the number of agents in the area of the shared space around the ego agent (including the ego agent) is a time varying variable $N^t$. The input at each time step can be denoted as $\mathbf{X}_i^t=(\mathbf{S}_a^t, \mathbf{I}_i^t)_{a=1}^{N^t}$, where $\mathbf{S}_a^t=(x_a^t, y_a^t, \dot{x}_a^t, \dot{y}_a^t)$ represents the state of the agent $a$, and $\mathbf{I}_i^t$ denotes the semantic map information at time $t$ around the ego agent. 

% In order to establish the interactions among the inputs, we first introduce the social force model. The social force model is defined by\cite{helbing1995social}:

% \begin{equation}\label{eq:socialforcephysics}
% \dfrac{d \vec{w}_i}{d t}:=\vec{F}_i(t)+fluctuations
% \end{equation}

% \begin{equation}\label{eq:originalsocialforceeqn}
% \begin{aligned} 
% \vec{F}_i(t) & :=\vec{F}_i^0\left(\vec{v}_i, v_i^0 \vec{e}_i\right)+\sum_R \vec{F}_{i R}\left(\vec{e}_i, \vec{r}_i-\vec{r}_R\right) \\ & +\sum_B \vec{F}_{iB}\left(\vec{e}_i, \vec{r}_i-\vec{r}_B^{\,i}\right)+\sum_A \vec{F}_{i A}\left(\vec{e}_i, \vec{r}_i-\vec{r}_A, t\right)
% \end{aligned}
% \end{equation}

% In equation \ref{eq:socialforcephysics}, $\vec{w}_i$ is the preferred velocity of pedestrian $i$. $\vec{F}_i(t)$ denotes the social force acting on the pedestrian $i$ at time $t$. $\vec{F}_i(t)$ can be written as the sum of four terms showed in equation \ref{eq:originalsocialforceeqn}: the acceleration term $\vec{F}_i^0$ which leads to a tendency to the desired speed $v_i^0$ and the desired direction $\vec{e}_i$, the repulsive force term of other pedestrians which is the sum of the force from each other pedestrian $R$ in a distance of $\vec{r}_i-\vec{r}_R$, the repulsive force term of borders summing up all effects from border $B$ with the shortest distance of $\vec{r}_i-\vec{r}_B^{\,i}$ to the pedestrian $i$ and the attractive force term coming from all the attractive persons or objects $A$ with the distance $\vec{r}_i-\vec{r}_A$ at time $t$. 

% Among the four terms of the social force, the acceleration term can be the result of the goal position which is the expected position of the pedestrian after a certain time in future. The actors of repulsive force and attractive force can be reclassified into two types: neighbor agents and static objects which can normally be represented in a semantic map. Then the social force can be written as the following form:

% \begin{equation}\label{eq:modifiedsocialforceeqn}
% \begin{aligned} 
% \vec{F}_i(t) &:=\vec{F}_i\left(G_i (t+\Delta t)\right) + \sum_N \vec{F}_{i N}\left(\vec{e}_i, \vec{r}_i-\vec{r}_N, t\right)  \\ &+ \sum_M \vec{F}_{i M}\left(\vec{e}_i, \vec{r}_i-\vec{r}_M^{\,i} , t\right)
% \end{aligned}
% \end{equation}

% The first term of equation \ref{eq:modifiedsocialforceeqn} is the goal force, $G_\alpha (t+\Delta t)$ represents the goal position of the pedestrian after time of $\Delta t$, the second is the neighbor force where $N$ is the neighbor agent, and the last term is the map force acted by semantic map object $M$. The last two terms depend on the direction $\vec{e}_i$ of pedestrian $i$, the relative state of the neighbors or objects, as well as the time. We propose our model based on the equation \ref{eq:modifiedsocialforceeqn}.

\subsection{Proposed model}
Our proposed model is composed of three main neural networks. It is visualized in fig. \ref{fig:fullnetwork}. The first network is a graph attention neural network encoding the social force acting on the ego agent from the observed history information. The second is a transformer encoder-decoder architecture to handle time sequence modelling. The history state sequence of the ego agent added with the social force serves as input for the transformer encoder, while the decoder yields the anticipated future embedding sequence. Finally, we integrate a CVAE generative model to produce multi-modal future trajectories of the ego agent based on the generated future embedding sequence. 


% \begin{figure*}[t!]
%   \centering
%     \includegraphics[height=3cm]{example-image-a}
%     \caption{This is the explanation for our network}
%     \label{fig:fullnetwork}
% \end{figure*}


% \begin{figure*}[!ht]
%   \centering
%   \begin{subfigure}[b]{0.8\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/social_force_embedding.pdf}
%     \caption{This is the social force embedding network architecture}
%     \label{fig:socialforceembedding}
%   \end{subfigure}
%   \begin{subfigure}[b]{1.0\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/generative_model.pdf}
%     \caption{This is the generative model architecture}
%     \label{fig:generativemodel}
%   \end{subfigure}
%   \caption{This is the explanation for our network}
%   \label{fig:fullnetwork}
% \end{figure*}

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.5\textwidth]{figures/network_diagram_rotated.pdf}
  \caption{GSGFormer model overview. Consider various VRUs in a structured urban environment, in BEV as shown. Our model uses the understanding of the interplay of social forces between different VRUs and the environment in which the motion is captured. A map encoder captures the influence of the environment on the VRU under consideration while the other encoders - for encoding the ego motion of the VRU, identifying the different goals of this VRU and those of its neighbours - are fed into a Graph Attention Network Encoder to capture a ``Social Embedding'' within the environment. Social Embeddings for each time step are then passed on to the Generative Phase of the model, where different contexts from the Transformer Decoder and the CVAE Encoder are concatenated along the last dimension of the tensor and passed to the Residual GMM generator. Finally, positions for a time interval $h$ from current time $t$ are predicted by integrating these velocities over the time interval $dt$. Best viewed zoomed in.}
  \label{fig:fullnetwork}
\end{figure}

\subsubsection{Agent State Encoder}
We classify the agent to four classes: pedestrian, bicycle, car, bus and trucks. The state of each class of the ego agent is embedded by a corresponding linear layer. The state of neighbors for the ego agent is converted to the ego-centric coordinate as \cite{jia2022hdgt} to represent the relative state of them to the ego agent. The neighbor state in a ego-centric view is embedded in the same way as the ego agent with a linear layer distinguished by the agent class. The output size of the agent state encoder is denoted as $d_{model}$.


\subsubsection{Map Encoder}\label{subsec:mapenc}

% The semantic segmentation model is inspired by the work done by Mangalam, Karttikeya and An, Yang and Girase, Harshayu and Malik, Jitendra for the Ynet model \cite{lee2017desire}.
To encode the map image, we first use a semantic segmentation U-Net\cite{ronneberger2015unet}-based model inspired by Y-Net\cite{mangalam2021goals} to get the semantic mask of the map RGB image.

% \paragraph{Architecture}
% The model uses the Unet architecture. Unet is a popular approach in semantic segmentation task because of its performance on small datasets. 
% It was developed by Olaf Ronneberger, Phillip Fischer,and Thomas Brox in 2015 for biomedical image segmentation \cite{ronneberger2015unet}.
% It is a U-shaped encoder-decoder network and in this work, we use a Resnet-101 encoder pretrained on Imagenet.  

% % \begin{figure}[!ht]
% %   \centering
% %   \includegraphics[width=0.5\textwidth]{figures/u-net-architecture.png}
% %   \caption{U-net architecture (example for 32x32 pixels in the lowest resolution).}
% %   \label{fig:unet}
% % \end{figure}

% \paragraph{Loss function}
% Multiple loss function were tested (Dice, Focal and Jaccard) and we got the best results using the Dice loss function.
% \begin{equation}\label{eq:diceloss}
%   \begin{split} 
%     DL(y,\hat{p}) & =  1 - \frac{2y\hat{p}+1}{y+\hat{p}+1} \\
%     & = 1 - \frac{2TP}{2TP + FP + FN}
%   \end{split}
% \end{equation}

% \paragraph{Data}
% In the Ynet paper, the authors trained 2 semantic segmentation models: one for the Sdd dataset and one for InD. In this work, we decided to create a single model using SDD, Ind and OpenDD datasets. 
% The SDD dataset consists of 8 unique locations that contains multiple videos. The videos of a given location do not cover the exact same region but might partially overlap. A scene image is provided for each video.  
% The Ind dataset contains 4 unique locations of German intersections and the OpenDD dataset 7 unique locations of German roundabounts. 

% \begin{table}[!ht]
% \begin{center}
%   \begin{tabular}{||c c c c||} 
%    \hline
%    Dataset & Situation &  \# of locations &  \# of scenes \\ [0.5ex] 
%    \hline\hline
%    SDD & Campus & 8 & 47  \\ 
%    \hline
%    InD & Intersections & 4 & 4  \\
%    \hline
%    OpenDD &Roundabounts & 7 & 7  \\
%    \hline

%   \end{tabular}
%   \caption{Locations and scenes of each datasets}
%   \label{table:1}
%   \end{center}
% \end{table}

The semantic masks were manually annotated in 6 classes as in \cite{mangalam2021goals}. In addition to the SDD\cite{robicquet2016learning} and inD\cite{inDdataset} datasets in the work\cite{mangalam2021goals}, we also used map images and our own segmentation annotations from the OpenDD dataset\cite{breuer2020opendd} as training set.
The segmentation examples are shown in Fig. \ref{fig:masks}.
% \begin{table}[!ht]
%   \begin{center}
%     \begin{tabular}{||c c||} 
%      \hline
%      Value & Class \\ [0.5ex] 
%      \hline\hline
%      0 & Background \\ 
%      \hline
%      1 & Pavement  \\
%      \hline
%      2 & Road \\
%      \hline
%      3 & Structure \\
%      \hline
%      4 & Terrain \\
%      \hline
%      5 & Tree \\
%      \hline
  
%   \end{tabular}
%   \caption{List of semantic classes}
%   \label{table:2}
%   \end{center}
% \end{table}

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.5\textwidth]{figures/images_masks_resized.png}
  \caption{Examples from the inD, SDD and OpenDD dataset. Above is the original image and below is the segmentation mask.}
  \label{fig:masks}
\end{figure}


% \paragraph{Data preprocessing}

% The final dataset contains 58 images randomly split between train and tests set with a ratio of 0.8. 
% All the images are resized to a width of 505 and a height of 355 and randomly cropped to (256,256) as the U-net architecture requires that the input size is a multiple of 32.  

% \begin{table}[!ht]
%   \begin{center}
%     \begin{tabular}{||m{1cm} m{1cm} m{1cm} m{1cm} m{1cm} m{1cm}||} 
%      \hline
%      Dataset & Similar sizes for all scenes & Min width & Maw width & Min height & Max height \\ [0.5ex] 
%      \hline\hline
%      InD & Yes & 780 & 780 & 1170 & 1170 \\ 
%      \hline
%      OpenDD & Yes & 2160 & 3840 & 2160 & 3840  \\
%      \hline
%      SDD & No & 741 & 2019 & 1184 & 1983 \\
%      \hline
  
%   \end{tabular}
%   \caption{Size of scene images}
%   \label{table:3}
%   \end{center}
% \end{table}

% Data augmentation is performed on the training set. Here are a few examples of the transformations done: 
% \begin{itemize}
%   \item Flipping 
%   \item Adding gaussian noise
%   \item Applying Contrast Limited Adaptive Histogram Equalization 
%   \item Changing brightness and contrast 
%   \item Blurring
%   \item Changing , saturation and value
% \end{itemize}


% Each transformation is associated with a probability of applying that augmentation to input data. 

% \paragraph{Training}

% \begin{table}[!ht]
%   \begin{center}
%     \begin{tabular}{||c c|} 
%      \hline
%      Parameter & Value\\ [0.5ex] 
%      \hline\hline
%      Learning rate & 0.001 \\ 
%      \hline
%      Training batch size & 8  \\
%      \hline
%      Validation batch size & 4  \\
%      \hline
%      Weight decay & ?  \\
%      \hline
%      Threshold & ?  \\
%      \hline
%      Epochs & ?  \\
%      \hline
%   \end{tabular}
%   \caption{Training parameters}
%   \label{table:4}
%   \end{center}
% \end{table}

% The table \ref{table:4} shows the hyperparameters used for training. The tuning was done using the Optuna framework. Moreover, we froze the Resnet101 encoder for the first 200 epochs, similarely to Ynet.

% \paragraph{Results}
% The performance of the model is evaluated using the Intersection Over Union (IoU score, also called Jaccard Index). The score is computed for each image and then averaged over the dataset.  

% \begin{equation}\label{eq:iou}
%   \begin{split} 
%     IoU & =  \frac{\text{Area of overlap}}{\text{Areaof Union}} \\
%     & = \frac{TP}{TP + FP + FN}
%   \end{split}
% \end{equation}

The segmentation mask output from the pre-trained segmentation model containing the semantic information is then encoded by a hand-designed 2D convolutional neural network (CNN) to the final map embedding.

\subsubsection{Goal Encoder}

We apply a 1D convolutional neural network to estimate the goal position. Initially, The state of the ego agent for each history time step is embedded using the agent state encoder. Then the embedding is stacked over the time dimension, resulting in a tensor of shape $(n \times d_{model})$. The 1D convolutional neural network extracts the temporal feature between the $n$ channels(time steps). The map embedding is concatenated to the output of the goal encoder and passed to a linear layer. The output of the network is a vector of size $d_{model}$. The vector then serves as the input condition for the CVAE-Residual-GMM module detailed further in \ref{subsec:cvaegmm}, facilitating the generation of a range of potential goals.

\subsubsection{Social Graph Attention Neural Network}

To model the social force acting on the ego agent, we introduce a heterogeneous graph representation. This representation comprises four distinct nodes: the ego agent, neighboring agents, the semantic map, and the goal. The node features are represented by the previously mentioned embedding vectors. For each time step and ego agent, we construct an undirected graph. Only the ego agent node is directly linked to the neighboring agent nodes, semantic map nodes, and goal nodes for that specific time step, as we focus solely on the social force's impact on the ego agent. Then a heterogeneous graph attention network\cite{wang2019heterogeneous} performs both node-level and semantic-level attention aggregating the social information to the ego agent node. The output is the social force embedding in size of $d_{model}$ is embedded from the aggregated ego agent node. 

Drawing inspiration from Newton's second law, we interpret the graph neural network's output as a force influencing the ego agent. This force is then element-wise combined with the state embedding of the ego agent, producing the social embedding for that particular time step.

\subsubsection{Temporal Transformer Model}  

Once the social information are encoded from the social graph of the ego agent at each time step, it is necessary to build the dependencies between graphs across different time steps. We employ a Transformer framework \cite{vaswani2017attention} to model the temporal relationship. The history sequence of social embedding are fed into the Transformer encoder as the source sequence with a fixed length n. Since the primary operation in Transformer is the attention mechanism which is not sensitive to the relative or the absolute position of the elements in the sequence, we add the "positional encodings" with the same dimension to each social embedding in the sequence. We compute positional encodings through sine and cosine functions, as described in \cite{vaswani2017attention}, which allows the model to easily learn to attend by relative positions. Meanwhile, it enables the model recognize any missing observations, as each comes with its distinct positional encoding.

The Transformer encoder processes the history sequence in parallel and outputs the memory providing the query for each observation time step. The Transformer decoder takes the embedded future ego agent's state sequence as the target sequence. The query of the memory is used to calculate the cross attention between the history sequence and future sequence. From the Transformer decoder, we obtain the predicted embedding sequence. Every embedding within this sequence serves as a condition for the waypoint CVAE-Residual-GMM Module (see in \ref{subsec:cvaegmm}), generating multi-modal states for each prediction horizon.


\subsubsection{CVAE-Residual-GMM Module}\label{subsec:cvaegmm} 

We propose a generative CVAE-Residual-GMM Module to realize the one-to-many mapping for both goal and waypoints. The module is composed of two main parts: a Conditional Variational Auto-Encoder(CVAE) \cite{sohn2015learning} and a Gaussian Mixture Model(GMM) \cite{dempster1977maximum}.  Let's denote the input condition as $\mathbf{X}$ and its corresponding output (be it goal position or waypoint state) as $\mathbf{Y}$. The high dimensional latent variable $\mathbf{Z}$ is drawn from the prior distribution $P_\theta(\mathbf{Z}|\mathbf{X})$, facilitated by a prior network. Throughout the training phase, given that the ground truth is accessible, $\mathbf{Z}$ is drawn from the posterior distribution $Q_\phi(\mathbf{Z}|\mathbf{X}, \mathbf{Y})$ by the recognition network. $\mathbf{Y}$ is finally generated from the distribution $P_\psi(\mathbf{Y}|\mathbf{X}, \mathbf{Z})$ through the generation network. 

Different from the vanilla CVAE, the generated $\mathbf{Y}$ is the sum of two parts: the output $\mathbf{\hat Y}$ from CVAE decoder decoding the concatenated $(\mathbf{X}, \mathbf{Z})$ and the residual $\mathbf{\Delta Y}$, which adheres to a GMM distribution. This distribution is parameterized by an MLP, defining means, variances, and component weights based on $(\mathbf{X}, \mathbf{Z})$. Notably, every waypoint within a single trajectory utilizes a consistent $\mathbf{Z}$ for each sampling iteration.

\subsubsection{Training Strategy}
During training, the most recent historical state, alongside the entire future state sequence, is concurrently fed into the Transformer decoder. A subsequent masking is applied to speed up the training and to ensure predictions for time step $t$ rely solely on preceding time steps. The latent variable $\mathbf{Z}$ is drawn both from $P_\theta(\mathbf{Z}|\mathbf{X})$ and $Q_\phi(\mathbf{Z}|\mathbf{X}, \mathbf{Y})$.

For inference, the decoder first receives the most recent historical state, followed by an auto-regressive procedure. The Transformer decoder's output embedding is then fed into the CVAE as condition $\mathbf{X}$. The latent variable $\mathbf{Z}$ is sampled from the prior network $P_\theta(\mathbf{Z}|\mathbf{X})$. The predicted state is calculated by summing up the output from CVAE decoder and the residual sampled from $P_\psi(\mathbf{\Delta Y}|\mathbf{X}, \mathbf{Z})$. This predicted state is subsequently appended in the time dimension to the previous input of the Transformer decoder to forecast the next time step. Notably, all waypoints in a single trajectory utilize a consistent $\mathbf{Z}$ throughout the sampling phase. 

The predicted position is determined by integrating the displacement of each time step, which is computed using velocity and time intervals. This method has been demonstrated to be more precise than directly utilizing the predicted position, as supported by \cite{salzmann2020trajectron++}.

\subsubsection{Loss function}

The loss function consists of two components: the waypoint and the goal loss, both represented through the CVAE loss format. The CVAE loss is expressed as the negative empirical lower bound (ELBO) \cite{sohn2015learning}. While the aim of CVAE is to maximize the ELBO, due to our reliance on gradient descent methods for optimizing the neural network, we aim to minimize the negative ELBO, detailed as follows:

\begin{equation}\label{eq:lossfunction}
\begin{aligned}
\mathcal{L} = \mathcal{L}_{\text {waypoint}} + \mathcal{L}_{\text {goal}} \\
\end{aligned}
\end{equation}


\begin{equation}\label{eq:ELBO}
\begin{aligned}
\mathcal{L}_{\text {CVAE}}= & -\mathbb{E}_{Q_\phi(\mathbf{Z}|\mathbf{Y}, \mathbf{X})}\left[\log P_\psi(\mathbf{Y}|\mathbf{X}, \mathbf{Z})\right]\\ &+\operatorname{KL}\left(Q_\phi(\mathbf{Z}|\mathbf{Y}, \mathbf{X}) \| P_\theta(\mathbf{Z}|\mathbf{X})\right)
\end{aligned}
\end{equation}

where $P_\theta(\mathbf{Z}|\mathbf{X})$ and $Q_\phi(\mathbf{Z}|\mathbf{Y}, \mathbf{X})$ are derived from the normal distribution probability determined by the mean and variance as parameterized by prior network and recognition network. $P_\psi(\mathbf{Y}|\mathbf{X}, \mathbf{Z})$ corresponds to the residual probability $P_\psi(\mathbf{\Delta Y}|\mathbf{X}, \mathbf{Z})$, which adopts a GMM distribution probability. This is because $\mathbf{Y}$ is the sum of $\mathbf{\hat{Y}}$ and $\mathbf{\Delta Y}$, where $\mathbf{\hat{Y}}$ is deterministic.



==> sections/experiments.tex <==
%!TEX root = ../main.tex
\section{Experiments and Results} \label{sec:implementation}

\subsection{Datasets}

% The performance of our model is evaluated on three public trajectory datasets the intersection Drone dataset (inD)\cite{inDdataset}, the Stanford Drone Dataset (SDD)\cite{robicquet2016learning}, and ETH\cite{pellegrini2009you}/UCY\cite{lerner2007crowds} dataset. All of these datasets are in stationary bird's eye view.

% The inD Dataset contains 32 drone recordings of trajectories of road users belonging to 5 classes including pedestrian, bicycle, car, truck and bus at 4 German intersections. The raw data is sampled in 25Hz. We split the training set and test set according to \cite{bertugli2021ac}. Specifically, we treat the data of location 1 and 2 as the training set, location 3 as the validation set and location 4 as the test set.

% The SDD Dataset is a large scale dataset providing drone recordings in the university campus consisting of 8 unique scenes and 60 videos in total. 6 classes of agent including pedestrians, skateboarders, bicyclists, carts, cars, and buses are annotated, of which pedestrians and bicyclists made up the majority. The raw data is sampled in 30Hz. Data split follows the TrajNet split\cite{sadeghian2018trajnet} and the whole dataset split proposed in \cite{lee2017desire}.

% ETH/UCY is a classic dataset widely used for the evaluation for pedestrian trajectory prediction which contain only data of pedestrians with rich human-human interactions. The raw data is taken from \cite{gupta2018social}. The data is annotated in 2.5Hz. We follow the leave-one-out strategy as previous works\cite{alahi2016social} for evaluation.

We train and evaluate our model on three stationary BEV datasets - the intersection Drone (\textbf{inD}) Dataset \cite{inDdataset}, the Stanford Drone Dataset (\textbf{SDD}) \cite{robicquet2016learning} and the \textbf{ETH/UCY} Dataset \cite{pellegrini2009you,lerner2007crowds}. 

\textbf{inD} dataset contains 32 drone recordings of various VRU trajectories of 5 different classes (pedestrian, bicycle, car, truck and bus) in 4 different scenes at German intersections. The raw data is samples in 25Hz. Training and test sets are split based on previous work done \cite{bertugli2021ac} such that scenes 1 and 2 of the dataset are considered as training data, scene 3 to be the validation set and scene 4 as the test set. 

\textbf{SDD} is a similar drone dataset, with 60 recordings at 8 unique scenes in the Stanford university campus, each scene containing a mixture of 6 classes of VRUs (pedestrians, skateboarders, bicyclists, cars, cars and buses). The raw data is sampled at 30 Hz. The entire dataset is split in two specific ways - one proposed in TrajNet \cite{sadeghian2018trajnet} and another full split as in DESIRE \cite{lee2017desire}. 

\textbf{ETH/UCY} is a classic dataset widely used for the evaluation for pedestrian trajectory prediction which contain only data of pedestrians with rich human-human interactions. The raw data is extracted and annotated at 2.5Hz. We follow the leave-one-out strategy as presented in previous works for evaluation \cite{alahi2016social,gupta2018social}.

The first two datasets are more representative of scenarios that AVs can face in urban environments, especially in shared spaces than the classic ETH/UCY dataset. The background RGB frames in these datasets act as the maps for our model. In each dataset, we only concentrate on predicting trajectories of the pedestrian VRU class while utilizing the effects of the other VRU classes on these pedestrians. Another rationale for utilizing similar datasets is to investigate our model's robustness to different scenes and vantages. 

% \subsection{Experiment Settings}

% We set the number of observed time steps and to be 8, and predict 12 future time time steps with a $0.4s$ time step which means that we predict the trajectory in the next $4.8s$ from the observed $3.2s$. The setting is consistent with most of the previous works \cite{alahi2016social,gupta2018social,sadeghian2019sophie, salzmann2020trajectron++, xu2022socialvae}.


\subsection{Experimental Setup}
For each of the datasets chosen and all their corresponding scenes, we perform trajectory preprocessing as provided by OpenTraj tools \cite{amirian2020opentraj}. All VRU trajectories are sampled at 2.5Hz and velocities for these trajectories are calculated as $\Delta X |_{t}^{t+1} / \Delta t$ where $X$ represents the sampled position at time $t$ and $\Delta t$ is the sampling interval. Each observed partial trajectory lasts for 8 timesteps with a prediction horizon $h$ of 12 timesteps thus implying a medium term trajectory prediction window of $4.8s$, consistent with the baselines (\ref{subsec:basemetric}) chosen to compare against our work. 

For each trajectory, a distance of $15m$ (or equivalent) is chosen as an effective threshold for neighbour interactions while a crop patch of $10m$ (or equivalent) is chosen for map interaction for social embeddings. Parantheses imply an estimation from pixel space to cartesian space where direct measurements are unavailable in the dataset. 

The model is set up to be trained on a single NVIDIA RTX A6000 GPU with 48 GB VRAM. 

\subsection{Baselines and Metrics}\label{subsec:basemetric}

We compare our model with different baselines for different datasets, since not all of them are evaluated on all the datasets that we choose. We introduce some common ones here:

\textbf{Social GAN}\cite{gupta2018social}: Social GAN is one of the earliest works that focus on multi-modal trajectories prediction. They apply GANs(Generative Adversarial Nets) to generate multi-modal outputs. The generator is in LSTM-encoder-decoder connected by a social pooling module which used to aggregate the social interactions. The discriminator is a LSTM encoder to determine whether the result from the generator is correct. Since it is a classic, many previous works reimplemented it on different datasets. The result of Social-GAN on inD and SDD dataset is obtained from \cite{chiara2022goal}.

\textbf{ST-GAT}\cite{huang2019stgat}: ST-GAT is a classic work on human trajectory prediction which uses graph attention network to model human interactions. LSTM is applied to model the temporal feature of the pedestrians. The result of it on inD dataset is obtained from \cite{chiara2022goal}.

\textbf{Y-Net}\cite{mangalam2021goals}: Y-Net is U-Net based network predicting multi-modal trajectories. The goal heatmap is generated first from the history trajectory heatmap and the map segmentation mask. And then the predicted trajectories are generated based on the sampled goal position. The model achieves very good results in both short-term and long-term trajectory prediction tasks. 

\textbf{NSP-SFM}\cite{yue2022human}: NSP-SFM is a successful example of the convergence of physics and deep neural network. The social force theory is modelled by neural networks and CVAE is used to implement the generation of multi-modalities. It achieved the best results in state-of-the-art on both SDD and ETH/UCY datasets. 

Following most of the previous studies, we consider to use the Average Displacement Error (ADE) and Final Displacement Error (FDE) as the metric to evaluate the performance of our model. ADE is the average $l_2$ distance error for each time step between the predicted position and the ground truth, and FDE is the $l_2$ distance error for the final prediction time step. Since our model outputs multi-modal trajectories, we report the min over 20 errors $\text{minADE}_{20}$ and $\text{minFDE}_{20}$ proposed in \cite{gupta2018social} which are the minimum ADE and FDE among 20 sampled predictions.

\subsection{Implementation details}

Data preprocessing is based on the OpenTraj tools\cite{amirian2020opentraj}. All datasets are sampled or down-sampled in 2.5Hz. The velocity is calculated by dividing the displacement of each time step by the time step length. 
The threshold distance to find neighbors is 15m and the cropped semantic map is a square with the side length of 10m around the ego agent. We calculate the approximate pixel size by the estimated scale for the dataset with only real world coordinates.
The position and velocity is normalized first and the position is then centered to the last observation time step. 

The dimension of all embeddings, the $d_{model}$ is set to be 128. 

We use two graph attention layers with 128 neurons in mean aggregation and 4 heads for each layer.

For Transformer module, the feed forward dimension is set to be 256. We use a single transformer encoder and decoder layer and 4 heads for the multi-head attention.

Each MLP for CVAE encoder, decoder and GMM has two hidden layers with 512 and 256. The dimension of the latent variable is 16 for the goal and 32 for the waypoint. The number of mixture components is set to be 4 for goal and 20 waypoint.

The model is trained on a single NVIDIA RTX A6000 with Adam optimizer. The learning rate is decayed every 10 epochs by a factor of 0.5. The model is trained for a total of 50 epochs with the batch size of 512.

\subsection{Quantitative Results}

\textbf{inD dataset.} Table \ref{table:ind} shows the the quantitative results on the inD dataset. We apply the evaluation protocol proposed in \cite{bertugli2021ac}. The benchmark is proposed in \cite{chiara2022goal}. 
We observe that our model has the lowest $\text{minADE}_{20}$ and the second lowest $\text{minFDE}_{20}$ among all showed models.

\begin{table}[!ht]
    \centering
    \normalsize
    \begin{tabular}{c|cc}
        \hline Method & $\text{minADE}_{20}$ & $\text{minFDE}_{20}$ \\
        \hline Social-GAN\cite{gupta2018social} & 0.48 & 0.99 \\
        ST-GAT\cite{huang2019stgat} & 0.48 & 1.00 \\
        AC-VRNN\cite{bertugli2021ac} & 0.42 & 0.80 \\
        Y-net*\cite{mangalam2021goals} & 0.34 & 0.56 \\
        Goal-SAR\cite{chiara2022goal} & 0.31 & \textbf{0.54} \\
        \hline
        GSGFormer(Ours) & \textbf{0.30} & 0.55 \\
        \hline
    \end{tabular}
    \caption{$\text{minADE}_{20}$ and $\text{minFDE}_{20}$ evaluated on the inD dataset in meters. Lower is better. Bold numbers indicate best. * indicates the Y-Net\cite{mangalam2021goals} result is trained by \cite{chiara2022goal}.}
    \label{table:ind}
\end{table}

\textbf{SDD.} Table \ref{table:sdd} shows the the quantitative results on the SDD dataset. We find that our model work best in the entire dataset but is not so good as the other models on the TrajNet split. 
We infer that it might because that the TrajNet split samples the trajectories without overlapping, which means there are not enough data for the model to learn the impact of the social force and our model needs more data to perform as well as the other models.


\begin{table}[!ht]
    \centering
    \normalsize
    \begin{tabular}{c|cc}
        \hline Method & $\text{minADE}_{20}$ & $\text{minFDE}_{20}$ \\
        \hline Social-GAN\cite{gupta2018social} & 27.25 & 41.44 \\
        Desire\cite{lee2017desire} & 19.25 & 34.05 \\
        SimAug\cite{liang2020garden} & \textbf{10.27} & 19.71 \\
        P2T\cite{deo2020trajectory} & 10.97 & 18.40 \\
        GSGFormer(Ours) & \textbf{10.27} & \textbf{16.67} \\
        \hline PECNet\cite{mangalam2020not} & 9.96 & 15.88 \\
        P2T\cite{deo2020trajectory} & 8.76 & 14.08 \\
        Y-Net\cite{mangalam2021goals} & 7.34 & 11.53 \\
        NSP-SFM\cite{yue2022human} & \textbf{6.52} & \textbf{10.61} \\
        GSGFormer(Ours) & 9.62 & 15.29 \\
        \hline
    \end{tabular}
    \caption{$\text{minADE}_{20}$ and $\text{minFDE}_{20}$ evaluated on the entire SDD dataset(above) and the TrajNet split(below) in pixels. Lower is better. Bold numbers indicate best}
    \label{table:sdd}
\end{table}

\textbf{ETH/UCY.} Table \ref{table:eth/ucy} shows the the quantitative results on the ETH/UCY dataset. Our model does not perform as well as the other models on this dataset. 
We think that it might because that the ETH/UCY dataset contains only pedestrians and the social force is not so strong as the other datasets. Meanwhile, the scene of ETH/UCY dataset is relatively simple and the semantic map is not so necessary for the prediction.

% \begin{table*}[!ht]
%     \centering
%     \normalsize
%     \begin{tabularx}{\textwidth}{ >{\centering\arraybackslash}X| >{\centering\arraybackslash}X| >{\centering\arraybackslash}X| >{\centering\arraybackslash}X| >{\centering\arraybackslash}X| >{\centering\arraybackslash}X| >{\centering\arraybackslash}X}
%         \hline \multicolumn{7}{c}{ Evaluation Metrics ($\text{minADE}_{20}$ $\downarrow /$ $\text{minFDE}_{20}$ $\downarrow$ )} \\
%         \hline Method& ETH & HOTEL & UNIV & ZARA1 & ZARA2 & AVERAGE \\
%         \hline Social-GAN\cite{gupta2018social} & 0.81/1.52 & 0.72/1.61 & 0.60/1.26 & 0.34/0.69 & 0.42/0.84 & 0.58/1.18 \\
%         \hline ST-GAT\cite{huang2019stgat} & 0.65/1.12 & 0.35/0.66 & 0.52/1.10 & 0.34/0.69 & 0.29/0.60 & 0.43/0.83 \\
%         \hline Transformer-TF\cite{giuliari2021transformer} & 0.61/1.12 & 0.18/0.30 & 0.35/0.65 & 0.22/0.38 & 0.17/0.32 & 0.31/0.55 \\
%         \hline Y-Net\cite{mangalam2021goals} & 0.28/0.33 & 0.10/0.14 & 0.24/0.41 & 0.17/0.27 & 0.13/0.22 & 0.18/0.27 \\
%         \hline NSP-SFM\cite{yue2022human} & \textbf{0.25}/\textbf{0.24} & \textbf{0.09}/\textbf{0.13} & \textbf{0.21}/\textbf{0.38} & \textbf{0.16}/\textbf{0.27} & \textbf{0.12}/\textbf{0.20} & \textbf{0.17}/\textbf{0.24} \\
%         \hline GSGFormer(Ours) & 0.56/0.99 & 0.18/0.31 & 0.32/0.56 & 0.21/0.35 & 0.16/0.28 & 0.29/0.50 \\
%         \hline
%     \end{tabularx}
%     \caption{$\text{minADE}_{20}$ and $\text{minFDE}_{20}$ evaluated on ETH/UCY dataset in meters. Lower is better. Bold numbers indicate best}
%     \label{table:eth/ucy}
% \end{table*}

\begin{table*}[!ht]
  \centering
  \normalsize
  \begin{tabular}{p{3.3cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}|p{1.8cm}}
      \hline \multicolumn{7}{c}{ Evaluation Metrics ($\text{minADE}_{20}$ $\downarrow /$ $\text{minFDE}_{20}$ $\downarrow$ )} \\
      \hline Method& ETH & HOTEL & UNIV & ZARA1 & ZARA2 & AVERAGE \\
      \hline Social-GAN\cite{gupta2018social} & 0.81/1.52 & 0.72/1.61 & 0.60/1.26 & 0.34/0.69 & 0.42/0.84 & 0.58/1.18 \\
      \hline ST-GAT\cite{huang2019stgat} & 0.65/1.12 & 0.35/0.66 & 0.52/1.10 & 0.34/0.69 & 0.29/0.60 & 0.43/0.83 \\
      \hline Transformer-TF\cite{giuliari2021transformer} & 0.61/1.12 & 0.18/0.30 & 0.35/0.65 & 0.22/0.38 & 0.17/0.32 & 0.31/0.55 \\
      \hline Y-Net\cite{mangalam2021goals} & 0.28/0.33 & 0.10/0.14 & 0.24/0.41 & 0.17/0.27 & 0.13/0.22 & 0.18/0.27 \\
      \hline NSP-SFM\cite{yue2022human} & \textbf{0.25}/\textbf{0.24} & \textbf{0.09}/\textbf{0.13} & \textbf{0.21}/\textbf{0.38} & \textbf{0.16}/\textbf{0.27} & \textbf{0.12}/\textbf{0.20} & \textbf{0.17}/\textbf{0.24} \\
      \hline GSGFormer(Ours) & 0.56/0.99 & 0.18/0.31 & 0.32/0.56 & 0.21/0.35 & 0.16/0.28 & 0.29/0.50 \\
      \hline
  \end{tabular}
  \caption{$\text{minADE}_{20}$ and $\text{minFDE}_{20}$ evaluated on ETH/UCY dataset in meters. Lower is better. Bold numbers indicate best}
  \label{table:eth/ucy}
\end{table*}

From this part, we can conclude that our model performs better on the large-scaled dataset with more complex scenes and more social force.

\subsection{Qualitative Results}

Figure \ref{fig:visualization} shows the visualization of the prediction result of multi-agent cases on the inD dataset and SDD dataset. We can see that in these cases, 
our model can predict the future trajectory of the multiple agents accurately. 

Figure \ref{fig:indbesttraj} and \ref{fig:indriskmap} show a case on the inD dataset. The heatmap of the distribution of the predicted trajectory
in future horizons can be used as the risk map for autonomous vehicles to evaluate the collision risk of the area. 

From Figure \ref{fig:sddbesttraj} and \ref{fig:sddriskmap}, we can see that our model also performs quite well on the SDD dataset. In this scenario, the future trajectories of almost all pedestrians are accurately predicted.

Heatmap in Figure \ref{fig:straight} and \ref{fig:turn} is the distribution of the predicted goal position of the ego pedestrian.
The red crosses are the sampled goal positions from the predicted goal distribution. We find each sample guides the trajectory to the goal position even there is no hard constraint making sure that the endpoint of the trajectory be the sampled goal.
By comparing two cases, we can see that the straight history trajectory leads to a concentrated distribution of the goal position in front of the ego agent, 
while the turning history trajectory will lead to a less confident goal position distribution.
We sampled the right goal position in both cases, which proves the effectiveness of our model in dealing with different cases.

\begin{figure*}[!ht]
  \centering
  \begin{subfigure}[b]{0.20\textwidth}
    \begin{minipage}[b]{1.0\textwidth}
      \includegraphics[width=\textwidth]{figures/best_traj.png}
      \caption{Best of 20 result(inD)}
      \label{fig:indbesttraj}
      \includegraphics[width=\textwidth]{figures/risk_map.png}
      \caption{Risk map(inD)}
      \label{fig:indriskmap}
    \end{minipage}
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/sdd_best_traj.png}
    \caption{Best of 20 result(SDD)}
    \label{fig:sddbesttraj}
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/sdd_risk_map.png}
    \caption{Risk map(SDD)}
    \label{fig:sddriskmap}
  \end{subfigure}
  \begin{subfigure}[b]{0.20\textwidth}
    \begin{minipage}[b]{1.0\textwidth}
      \includegraphics[width=\textwidth]{figures/case_straight.png}
      \caption{Straight trajectory case}
      \label{fig:straight}
      \includegraphics[width=\textwidth]{figures/case_turn.png}
      \caption{Turning trajectory case}
      \label{fig:turn}    
    \end{minipage}
  \end{subfigure}
  \caption{Visualization of the prediction result on the inD dataset(a), (b), (d) and (e), the SDD dataset(c) and (d). (a) and (c) are the best of 20 prediction. (b) and (d) are the generated risk map. The red trajectory is the ground truth, the yellow trajectory is the prediction result and the magenta trajectory is the observed trajectory. The overlapped heatmap of the predicted trajectories for each pedestrian can be seen as the risk map on the road. Heatmaps in (e) and (f) are the predicted goal position distribution of the pedestrian in two cases of straight and turning history trajectories. Red crosses are the sampled goals and yellow scatters are sampled trajectories.}
  \label{fig:visualization}
\end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \begin{subfigure}[b]{0.24\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/best_traj.png}
%       \caption{Best of 20 result(inD)}
%       \label{fig:indbesttraj}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/risk_map.png}
%       \caption{Risk map(inD)}
%       \label{fig:indriskmap}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/sdd_best_traj.png}
%       \caption{Best of 20 result(SDD)}
%       \label{fig:sddbesttraj}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/sdd_risk_map.png}
%       \caption{Risk map(SDD)}
%       \label{fig:sddriskmap}
%     \end{subfigure}
%     \caption{Visualization of the prediction result on the inD dataset. (a) is the best of 20 prediction and (b) is the generated risk map. The red trajectory is the ground truth, the yellow trajectory is the prediction result and the magenta trajectory is the observed trajectory. The risk map is the overlapped heatmap of the predicted trajectories for each pedestrian.}
%     \label{fig:indresult}
% \end{figure*}

% \begin{figure*}[!ht]
%   \centering
%   \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/sdd_best_traj.png}
%     \caption{Best of 20 result(SDD)}
%     \label{fig:sddbesttraj}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/sdd_risk_map.png}
%     \caption{Risk map(SDD)}
%     \label{fig:sddriskmap}
%   \end{subfigure}
%   \caption{Visualization of the prediction result on the SDD dataset. (a) is the best of 20 prediction and (b) is the generated risk map. The red trajectory is the ground truth, the yellow trajectory is the prediction result and the magenta trajectory is the observed trajectory. The risk map is the overlapped heatmap of the predicted trajectories for each pedestrian.}
%   \label{fig:sddresult}
% \end{figure*}


  % \begin{figure*}[!ht]
  %   \centering
  %   \begin{subfigure}[b]{0.3\textwidth}
  %     \begin{minipage}[b]{0.3\textwidth}
  %       \includegraphics[width=1\textwidth]{figures/case_straight.png} \\
  %       \includegraphics[width=1\textwidth]{figures/case_turn.png}
  %     \end{minipage}
  %   \end{subfigure}
       
      
  %   %   \centering
  %   %   \includegraphics[width=\textwidth]{figures/case_straight.png}
  %   %   \caption{Straight trajectory case}
  %   %   \label{fig:straight}
  %   % \end{subfigure}
  %   % \begin{subfigure}[b]{0.3\textwidth}
  %   %   \centering
  %   %   \includegraphics[width=\textwidth]{figures/case_turn.png}
  %   %   \caption{Turning trajectory case}
  %   %   \label{fig:turn}
  %   % \end{subfigure}
  %   \caption{Case study for straight(a) and turning(b) history trajectory case. Heatmap is the predicted goal position distribution. Red crosses are the sampled goals and yellow scatters are sampled trajectories.}
  %   \label{fig:cases}
  % \end{figure*}


\subsection{Ablation Study}

We perform the ablation study on the inD dataset to verify the effectiveness of each module that we propose. 
We start from the architecture without social force graph module and the residual GMM, where only the observed trajectory of the ego agent is input to the model and the output layer is a single CVAE trained by the $l_2$ loss of the waypoint but not the negative log likelihood loss. 

Then we add the residual GMM(RM), goal prediction(G), neighbor trajectories(N), and semantic map mask(S) step by step, we find that the metric ADE and FDE gradually decline with the addition of each module which proves that the each component of our proposed module makes an important role in the prediction.
We notice that the addition of Residual GMM module reduces ADE and FDE by around 50 percent.


\begin{table}[!ht]
    \centering
    \normalsize
    \begin{tabular}{cccc|cc}
    \hline RG & G & N & S & $\text{minADE}_{20}$ & FDE \\
    \hline & & & & 0.58 & 1.31 \\
    $\checkmark$ & & & & 0.35 & 0.65 \\
    $\checkmark$ & $\checkmark$ & & & 0.31 & 0.57 \\
    $\checkmark$ & $\checkmark$ & $\checkmark$ & & 0.31 & 0.56 \\
    $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & \textbf{0.30} & \textbf{0.55} \\
    \hline
    \end{tabular}
    \caption{Ablation study result on inD dataset. RG: Residual GMM, G: Goal prediction, N: Neighbor trajectories, S: Semantic map mask. The tick indicates the module is added. $\text{minADE}_{20}$ and $\text{minFDE}_{20}$ are reported in meters.}
\end{table}





==> sections/related_work.tex <==
%!TEX root = ../main.tex
\section{Related Work} \label{sec:related_work}

\subsection{Sequence modelling}

A trajectory refers to a sequential sequence of positions in the dimension of time. Recurrent Neural Network (RNN), such as LSTM and GRU, is the mostly used neural network encoder to model temporal sequences. \cite{alahi2016social, salzmann2020trajectron++, huang2019stgat, gupta2018social, lee2017desire, vemula2018social}. Some other model such as Markov Model \cite{vasishta2018building}, Time-Extrapolator Convolution Neural Network (TXP-CNN) \cite{mohamed2020social}, U-Net \cite{mangalam2021goals} are also able to extract the temporal features from pedestrian trajectories.

Recently, the sequence model Transformer, which was originally proposed for NLP mission \cite{vaswani2017attention}, has also demonstrated the effectiveness in modelling trajectory sequence\cite{giuliari2021transformer,yuan2021agentformer,yu2020spatio, zhang2023forceformer}. Especially when it comes to situations where sensors lose data at a certain moment, which is likely to be encountered in real applications, the Transformer structure does not incorrectly determine the relative temporal relationship of the signals due to its positional coding properties, which is difficult for RNNs to deal with.


\subsection{Social forces modelling}

The concept of social force was explained and applied to describe human behaviors by \cite{helbing1995social}. It is the motivation that drives individuals to act and produce acceleration or deceleration forces in response to the information they perceive about their environment. The actor of social forces can be classified into three categories: neighbor agents, static objects or information that can be represented on a map such as road, sidewalk, and the goal position of the ego agent. 

Social pooling \cite{alahi2016social, gupta2018social}, attention mechanism \cite{vemula2018social, sadeghian2019sophie, xu2022socialvae} and graph representation or graph neural network \cite{huang2019stgat, yu2020spatio, xu2023eqmotion} are three common ways to model neighbor interactions in previous studies. \cite{mo2022multi,chiara2022goal} applied the heterogeneous graph network to model the interaction between different type of nodes. 

For the static objects that can be represented in a semantic map, it can help to find the attractive and repulsive potential fields in the scene\cite{vasishta2017natural}. Embedding the entire map into a vector using an encoder, which is then spliced to predict the feature vector of the ego agent at each time step has been widely used \cite{salzmann2020trajectron++, yuan2021agentformer, messaoud2021trajectory}. \cite{sadeghian2019sophie} utilizes a physical attention to take in account the map information. 

In addition, the goal distribution can also be predicted with the aide of semantic map along with the history trajectory heatmap \cite{mangalam2021goals,chiara2022goal}, and the predicted goal guides the agent to the goal. Goal position prediction can also be based on the past observation signals but not the heatmap which cost fewer computing resources \cite{mangalam2020not, wang2022stepwise, yue2022human}.  

\subsection{Multi-modal output}   

Considering the human behavior is stochastic, to handle the uncertainty, it's necessary to make multi-modal predictions. A Best-of-N metric is first proposed by \cite{gupta2018social}, and is used to evaluate the performance of the model in most of the multi-modal trajectory prediction works. Noise-based framework is widely used to generate diverse samples. A simple random noise is added or concatenate to the input of the decoder generating the trajectory in some works \cite{huang2019stgat, yu2020spatio}. \cite{gupta2018social, sadeghian2019sophie} use GAN adding adversarial loss to generate prediction with higher quality. CVAE model has been popular to implement multi-modal trajectory prediction \cite{lee2017desire, salzmann2020trajectron++, yuan2021agentformer, xu2022socialvae, yue2022human} due to its ability to learn the latent variable distribution from the prior condition. To explicitly express different modalities, certain anchor conditioned methods have been proposed\cite{huang2023multimodal}, such as predicted endpoint conditioned (PEC)\cite{mangalam2020not} and prototype trajectory conditioned (PTC)\cite{kothari2021interpretable} framework to encourage more explainable predictions. In addition, some grid-based approaches predicts the multi-modal occupancy grid map in each time step using specialized sample methods such as MaxEnt reinforcement learning policy\cite{deo2020trajectory}, Gumbel-Softmax trick \cite{guo2022end}.
 
